M-HOF-Opt: Multi-Objective Hierarchical Output Feedback Optimization via Multiplier Induced Loss Landscape Scheduling

A probabilistic graphical model is proposed, modeling the joint model parameter and multiplier evolution, with a hypervolume based likelihood, promoting multi-objective descent in structural risk minimization. We address multi-objective model parameter optimization via a surrogate single objective penalty loss with time-varying multipliers, equivalent to online scheduling of loss landscape. The multi-objective descent goal is dispatched hierarchically into a series of constraint optimization sub-problems with shrinking bounds according to Pareto dominance. The bound serves as setpoint for the low-level multiplier controller to schedule loss landscapes via output feedback of each loss term. Our method forms closed loop of model parameter dynamic, circumvents excessive memory requirements and extra computational burden of existing multi-objective deep learning methods, and is robust against controller hyperparameter variation, demonstrated on domain generalization tasks with multi-dimensional regularization losses.

==> abs_old_aistat.tex <==
When the loss function parameterized over a neural network constitutes many terms, as commonly found in Structural Risk Minimization (SRM) and domain generalization, the combinatorial choice of multipliers weighting each term greatly affects the performance. We propose a probabilistic graphical model (probabilistic graphical model) for the classical multiplier adaptation process, and interpret the model parameter estimation process as an optimal control problem. This leads us to design a dynamic system for the multiplier choice, along with the dynamics for the model parameters, which forms a hierarchical control structure. Via output feedback, a high level signal serves as a multi-objective setpoint for the low level controller, while automatically adapting itself according to Pareto dominance. The low level controller output updates the multipliers for the model parameter dynamic system.

Our method is multiplier free while only requiring a minimal number of hyperparameters. We applied our hierarchical controller to domain invariant variational auto-encoding on a domain generalization task, and observed stable performance across a range of hyperparameters, outperforming baseline methods.


==> authors_affi.tex <==
% Add authors
%\author[1]{\href{mailto:<jj@example.edu>?Subject=Your UAI 2024 paper}{Jane~J.~von~O'L\'opez}{}}

\author[1]{\href{mailto:<ac.xudong.sun@gmail.com, sun-xudong@outlook.com>?Subject=M-HOF-Opt}{Xudong~Sun}
\thanks{
\tiny{\tiny{ac.xudong.sun@gmail.com}\\ code: \url{https://github.com/marrlab/DomainLab/tree/mhof}}
} 
}
\author[2]{Nutan~Chen}
\author[3]{Alexej~Gossmann}
\author[4]{Yu~Xing}
\author[1]{Carla~Feistner
%$\;^\dag$
%\printfnsymbol{1}
}
\author[1]{Emilio~Dorigatti
%\thanks{\small{ED, CF, FD contributed equally}}
}
%\author[1]{Carla~Feistner$\;^*$

\author[1]{Felix~Drost
%$\;^\dag$
%\printfnsymbol{1}
}

%\footnotetext{These authors contributed equally to this work}
\author[1]{Daniele~Scarcella}
\author[1]{Lisa~Beer}
\author[1]{
%\href{mailto:<carsten.marr@helmholtz-munich.de>?Subject=M-HOF}
{Carsten~Marr}
%\thanks{\small{carsten.marr@helmholtz-munich.de}}
}
% Add affiliations after the authors
\affil[1]{\small Institute of AI for Health, Computational Health Center,  Helmholtz Munich, Munich, Germany}
\affil[2]{\small Machine Learning Research Lab,  Volkswagen Group, Munich, Germany}
\affil[3]{\small U.S. FDA Center for Devices and Radiological Health\\Silver Spring, MD, USA (former affiliation)}
\affil[4]{\small KTH Royal Instiute of Technology\\Stockholm\\Sweden}
%\affil[5]{test font normal}
%\affil[6]{\small test font small}
% \affil[5]{\small TUM\\Address\\}


==> caption_beta_y.tex <==
For the regularization loss of KL-divergence corresponding to multiplier $\beta_y$ in ~\Cref{eq:loss_diva_beta_y}, we see that it starts with  a negative value (blue curve) with the setpoint set to $\rho = 99\%$ in \Cref{eq:setpoint_ini} of its initial value (red line), and that in the initial epochs the $R$ loss in ~\Cref{eq:loss_diva_beta_y} overshoot to an even worse value, but our controller pulls it back towards the setpoint in later epochs and keeps it oscillating around the setpoint with small error.

==> caption_loss_gamma_d.tex <==
For the domain classification loss corresponding to multiplier $\gamma_d$ in ~\Cref{eq:loss_diva_gamma_d} (blue curve), we observe that in the first few epochs the loss overshoots substantially, until our controller drags it back to be below the setpoint (red curve). After all constraints in \Cref{eq:feasibility_r} are satisfied (i.e., blue curve below red curve), the setpoint (red curve) also gets adapted as a new goal to be reached by the $R$ loss in \Cref{eq:loss_diva_gamma_d}.

==> caption_pgm_rfms_multi_datasite.tex <==
Probabilistic graphical model for Restrictive Federated Model Selection (RFMS): \input{caption_hyper_para_tune_bayes}\\
In remote data site, the data $X_{cu}$ is from the path $\beta \rightarrow D_{cu} \rightarrow X_{cu}$ and $Y_{cu}\rightarrow X_{cu}$. The only information  can get remote data site $D_{cu}$ is the performance estimator $S_{cu}$.


==> caption_recon.tex <==
For the regularization loss of VAE reconstruction in ~\Cref{eq:loss_diva_recon}, it is always decreasing, it satisfies our setpoint constraint all the time after a few epochs.

==> caption_rfms.tex <==
$\phi$ is hyper-parameter of machine learning algorithm $\mathcal{L}$, $J$ is local performance estimator computed through cross validation $cv$ in the figure, $\mathcal{F}$ is remote performance estimator. Multi-objective Bayesian optimization is responsible for learning the function $f(\phi_i|\phi_{i-1:1},J_{i-1:1}, F_{i-1:1})$ for efficient search of hyper-parameter $\phi$. The search index is $i$.


==> conj_pareto_descent_generalize.tex <==
\begin{conj}
The fundamental conjecture of this paper is that a Pareto (multi-objective) descent of both $\ell(\cdot)$ and $R(\cdot)$ leads to a refined partition of the hypothesis space $\mathcal{H}$, where $\mathcal{H}$ is the collection of possible model parameters $\theta$. For brevity of discussion, we fix the neural network architecture. 
\end{conj}

==> def_pareto_slider.tex <==
\begin{definition}\label{def:reg-pareto-slider} 
A reg-Pareto slider $\mathcal{A}(\cdot)$ with respect to function $\ell(\cdot)$ and $R(\cdot)$ is defined to be a set map, s.t.~ if
$\{\theta^{(k+1)}, \bar{\theta}^{(k)}=\theta^{(k)}, \mu^{(k+1)}\} \in \mathcal{A}(\mathcal{\ell}(\cdot), R(\cdot);\theta^{(k)}, \mu^{(k)})$ then
\begin{align}
\ell(\theta^{(k+1)}) + \mu^{(k+1)} R(\theta^{(k+1)})&\le \ell(\bar{\theta}^{(k)}) + \mu^{(k+1)} R(\bar{\theta}^{(k)})\label{eq:improve_new_lambda}\\
\ell(\theta^{(k+1)}) + \mu^{(k)} R(\theta^{(k+1)})&\ge \ell(\bar{\theta}^{(k)}) + \mu^{(k)} R(\bar{\theta}^{(k)})\label{eq:deteriorate_old_lambda}\\
\mu^{(k+1)}&\ge \mu^{(k)} \label{eq:mu_increase}
\end{align}
If 
\begin{equation*}
\{ \theta^{(k+1)}, \bar{\theta}^{(k)}\neq \theta^{(k)}, \mu^{(k+1)}\} \in \mathcal{A}(\mathcal{\ell}(\cdot), R(\cdot);\theta^{(k)}, \mu^{(k)})   
\end{equation*}
the above equation should hold for $\theta^{(k)}$ taking the place of $\bar{\theta}^{(k)}$. 
\end{definition}
%\CF{In this definition you say that equations \cref{eq:improve_new_lambda} and \cref{eq:deteriorate_old_lambda} should hold for $\bar{\theta}^{(k)}$ if $\bar{\theta}^{(k)}=\theta^{(k)}$, if on the other hand $\bar{\theta}^{(k)}\neq\theta^{(k)}$ is should still hold for  $\theta^{(k)}$ taking the place of $\bar{\theta}^{(k)}$ (i.e. use $\bar{\theta}^{(k)}=\theta^{(k)}$). for me it now does not make any sense anymore why you do introduce $\bar{\theta}^{(k)}$ if you only use $\theta^{(k)}$.}


In this situation, take $R(\cdot)\in \mathbb{R}^{d=1}$, we have the following conclusion
\input{thm_pareto_slider}

\input{thm_ell_bound}

==> eq_ma_setpoint_adjust.tex <==
\begin{align}
O_R^{(k)} &= \xi_{o}O_R^{(k-1)} + (1-\xi_{o}) R^{(k)}\label{eq:output_ma}\\
r^{(k+1)} &=\xi_{r}r^{(k)} + (1-\xi_{r})O_R^{(k)}\label{eq:setpoint_ma}   
\end{align}
See \cref{fig:tensorboard_jigen_fbopt_ma0} when these moving average is not used which correspond to a staircase descent of setpoint and the tracking of the regularization loss is always behind the setpoint. 

\subsection{Choice of  $\xi_d$, $\xi_o, \xi_r$}
The moving average parameters take values between 0 and 1. An example of those hyperparameters can be $\xi_d=0.5, \xi_o=0.1, \xi_r=0.9$, 

where $\xi_d$ is the moving average parameter $\delta(\cdot)$ trading off between P (proportional) and I (integral) control, the bigger the $xi_d$, the more weight it put on previous errors.

$\xi_o$ controls the tradeoff of estimating the output state $O_R$, which can put more weight on current $R(\cdot)$

$\xi_r$ controls how fast one should decrease the setpoint.

==> fig_dataset_pacs.tex <==
%\begin{figure}[h!]
%\centering\includegraphics[width=0.65\linewidth]{tex/figs/mnist_te0tr12.png}\includegraphics[width=0.35\linewidth]{tex/figs/PACS.jpg}
    %\caption{\textbf{Left}: Domain generalization task with Colored MNIST dataset: We train on domain 1 and domain 2 and test on domain 0. Note that the training domain has color green and yellow while the test domain has color red and blue, so there is no color intersection, and this is not an easy task. \textbf{Right}: Domain generalization task with PACS dataset: We train on Pictures(P, last row), Art painting (A, first row), Cartoon(C, second row) and test on Sketch (S, third row)}
   %\label{fig:mnist_te0tr12}
%\end{figure}

==> fig_phase_portrait.tex <==
\begin{figure}[!htbp]
\centering
\includegraphics[width=0.9\linewidth]{figs/figs_diva_pacs_mhof_output_portrait/phase_portrait_R_gamma_d_pdfpage.eps}
\caption{Our training scheme adapts the multi-dimensional multiplier $\mu$, steering the optimization process towards a configuration that balances the trade-off between minimizing output $\ell(\cdot) = \mathbb{E}_{q_{\phi_y}(z_y|x)}[\log q_{\omega_y}(y|z_y)]$ in \Cref{eq:loss_diva_gamma_y} and 
%adhering to each of the regularization constraint (including the component plotted here). 
%A phase portrait inspired view of 
%output $\ell(\cdot)=\mathbb{E}_{q_{\phi_y}(z_y|x)}[\log q_{\omega_y}(y|z_y)]$ in \Cref{eq:loss_diva_gamma_y} (horizontal axis) and 
output $R_{\gamma_d}(\cdot)=\mathbb{E}_{q_{\phi_d}(z_d|x)}[\log q_{\omega_d}(d|z_d)]$ in~\Cref{eq:loss_diva_gamma_d}.
%corresponding to $\gamma_d$ (vertical axis) evolves as all multipliers in \Cref{eq:loss_diva_srm} are adaptively changing with \Cref{eq:pid} throughout the training process. 
In this plot, the solid large point corresponds to the initial output. We use gradually changing colors to indicate the training iterations (epochs), indicated by the color bar. 
%For better visualization, we only used the first 120 epochs and plot only every 10 epochs. 
For improved visualization, we exclusively utilized the initial 120 epochs and plotted data points solely for every 10 epochs. This figure corresponds to \Cref{fig:dyn_pacs_diva_fbopt}.
}\label{fig:phase_portrait_pacs_diva_fbopt}
\end{figure}


==> para_motivation_exp.tex <==
In \cite{gulrajani2020search}, the authors showed, when using Resnet50, ERM without any regularization term $R(\cdot)$ still pertains to a very competitive baseline with state-of-the-art performance. In our experiments in \Cref{sec:exp}, we also reaffirmed their findings, beyond which we observed that the studied domain generalization methods only achieve an expected generalization performance if the ``correct'' multipliers are used in front of the corresponding regularization losses in \Cref{eq:srm}. 

However, it is not obvious how those ``correct'' multipliers could be practically obtained when we lack information on the test domain distribution, in contrast to the classical hyperparameter tuning where we optimize hyperparameters to enhance the validation set prediction performance.   

This motivates our work in developing multiplier-free algorithms, where we defined dynamic systems for those multipliers and have those multipliers automatically adjusted according to output feedback of the corresponding losses. 

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec_abstract_old.tex <==
%Due to lack of theoretical underpinnings of the function property and limited data, the open loop behavior of this dynamic system is not guaranteed, which we coin an uncertain plant. 

An optimizer applied to a loss function parameterized over a neural network establishes a dynamic system over the model parameters.
Especially when the loss constitutes several terms, as commonly found in Structural Risk Minimization and domain generalization, the uncertainty of this dynamic system can become more pronounced with respect to a multi-objective descent for each loss term. 
Additionally, the combinatorial choice for the multipliers weighting each loss term greatly affects the performance, while the choice space grows dramatically with the addition of more regularization terms, making searching for an optimal combination challenging.
To alleviate these two issues, we propose a hierarchical controller to guide this dynamic system via output feedback from each loss term. 
A high-level signal serves as a multi-objective setpoint for the low-level controller, while automatically adapting itself according to Pareto dominance. The low-level controller updates the multipliers for the model parameter dynamic system. 

Our method is multiplier free while only admitting a minimal number of hyperparameters. We applied our hierarchical controller to domain invariant variational auto-encoding on a domain generalization task and observed stable performance with respect to varying hyperparameters compared to baselines.
%, which changes dramatically due to change of multiplier setting.

%The hierarchical collaboration of the high-level and low-level controllers drives the multi-objective loss towards its setpoint, which forms a constrained optimization problem, with its solution leading to a multi-objective model selection criterion. In addition, we further adapt the setpoint according to Pareto dominance, which forms the top hierarchy of the controller.  
%and found that the proposed approach circumvents the challenge of multiplier combination choice, while achieving stable competitive test domain generalization performance.   
%The loss of a deep neural network is implicitly defined over limited data, which can lead to overfitting to the training data distribution. 



%Considering that modern neural networks suffer greatly from distribution shift, domain generalization aims at training domain invariant neural networks for better generalization on unseen test domains, typically by appending penalty or regularization losses to boost cross-domain alignment. 


==> sec_app.tex <==

\onecolumn

\title{\mytitle \\(Supplementary Material)}
\maketitle

\appendix
\section{Visualizations for experimental results}
%The following includes visualizations for the experiments described in \Cref{sec:exp} .

\input{sub_sec_dg}
\input{sec_setpoint_model_sel}
% \input{sec_relatedwork}
\input{fig_phase_portrait}

\input{tex/sec_license}

\input{fig_hv_illustration}





% \begin{figure}
% \centering
% \includegraphics[width=0.9\linewidth]{tex/figs/jigen_mnist/fbopt_jigen_100_epo_ma0.png}
% \caption{Setpoint tracking behaviour when no moving average used in \Cref{eq:setpoint_ma} and \Cref{eq:output_ma}. Reproducibility: python main\_out.py --te\_d=0 --tr\_d 1 2 --task=mnistcolor10 --bs=16 --aname=jigen --trainer=fbopt --nname=conv\_bn\_pool\_2 --epos=2000 --es=5 --mu\_init=1e-6 --coeff\_ma\_setpoint=0 --coeff\_ma\_output\_state=0 --force\_setpoint\_change\_once --epos\_min=100}
% \label{fig:tensorboard_jigen_fbopt_ma0}
% \end{figure}

% \begin{figure*}[h!]
% \centering
% \includegraphics[width=0.45\linewidth]{tex/figs/jigen_mnist/timecourse_regularization loss jigen_setpoint.png}
% \includegraphics[width=0.45\linewidth]{tex/figs/jigen_mnist/phase_portrait_combined_regularization loss jigen.png}
% \caption{color-mnist: Using model Jigen~\cite{carlucci2019domain} with FBOPT: \textbf{Left}: the regularization loss of Jigen is tracking its setpoint. \textbf{Right}: Phase portrait of $\ell(\cdot)$ and $R(\cdot)$ in \Cref{eq:srm}, starting  with solid circle on the top right corner. We use arrow to indicate the direction of the change of $\ell(\cdot)$ and $R(\cdot)$, and to enhance visibility we iterate over 5 different colours in the scatter plot. 
% The classification loss $\ell(\cdot)$ first become larger (deteriorates) at initial epochs (corresponding to \Cref{def:reg-pareto-slider}), then decrease (improves) together with regularization loss (corresponding to \Cref{def:pareto-descent-operator}) until it enters a region where the evolution is not clear anymore (We make no theoretical analysis here). 
% %Dynamics of $\mu$ and its controller, output selected, test and validation accuracy, an error signal of the controller, output loss and their setpoints: the loss tracks the output. \\
% %First row: accuracy, second column is setpoint selected accuracy in \cref{sec:msel_setpoint}\\
% %Second row: the controller gain on multiplier\\
% %Third row: the delta signal in \cref{eq:delta_ma} \\
% %Fourth row: the time course (dynamics) of multiplier\\
% %Fifth row: the loss $R$ plotted together with setpoint\\
% %Sixth row: the task loss $\ell$ and penalized loss $ \ell(\cdot) + \mu R(\cdot)$
% %Note that our model selection in \Cref{sec:msel_setpoint} has smoothed out the selected model accuracy in the first row, to the end, the last setpoint it not reachable anymore so we only keep the last but 2nd selected model. (reproducibility: run\_fbopt\_mnist.sh)
% }
% \label{fig:tensorboard_mnist_jigen}
% \end{figure*}


==> sec_dg_basic.tex <==
\section{Pre-requisite}
\textbf{Meta Learning} Meta Learning train a model over multiple tasks, in order to generalize to a new task with few samples~\cite{finn2017model}. Model Agnostic Meta Learning \cite{finn2017model} trains the neural network through multiple tasks to make the parameters highly sensitive to the new task loss function, so few samples could lead to new task improvements. Few-Shot Meta Learning aims at training a model that can adapt to a new task through a few new instances and training iterations. 

\textbf{Transfer Learning, Domain Adaptation, Domain Generalization.} Transfer learning is the process of improving the target predictive function by using related information from the source domain. The domain adaptation process aims to alter a source domain in an attempt to bring the distribution of the source closer to that of the target~\cite{weiss2016survey}. Domain generalization is the process of utilizing data from several domains to train a system that generalizes to a previously unseen domain \cite{akuzawa2019adversarial}. JAN~\cite{long2017deep} and DAN~\cite{akuzawa2019adversarial} are two neural network architectures in the domain generalization field. 
\XS{We should investigate into JAN}
\XS{Nutan also mentioned we could first try to use the posterior of the first task, as the prior for the second task
	the idea is for the scenario that we can use the new dataset for training (it is not necessary to be labeled). 
}
As in Equation (\ref{eqn:dan}) and Figure~\ref{fig:dan}, classification network $M$ tries to improve classification, encoder $E$ tries to remove domain information, domain recognition network $D$ tries to recover domain information.
\begin{align}
	\underset{E,M}{min}\underset{D}{max} E\left[\underbrace{\gamma \log q_D(s\mid h=E(x,s))}_{\text{recognize domain from encoder}} \underbrace{- \log q_M(y \mid h=E(x,s))}_{\text{bad classfication}}\right]\label{eqn:dan}
\end{align}

\begin{figure}[H]
	\centering
	\includegraphics[scale=0.5]{fig/dan.png} 
	\caption{Architecture of DAN}
	\label{fig:dan}
\end{figure}


\textbf{Batch Normalization:} Batch Normalization \cite{ioffe2015batch} is a technique to reduce the distribution shift problem in training neural network.
\textbf{Zero-Shot Learning:} Suppose there are $S+U$ number of classes where $S$ class labels are seen during training. Each class label is represented by attribute vector of length $M$. At test time, unseen class instance is to be predicted. In \cite{wang2018zero}, the author define the class attribute vector as $a_n$ where $n$ is the instance index. To make a connection of the attribute vector with the density estimation model, the prior distribution parameter for $Z$ is determined by $a_n$ through a linear function, so one could write the prior distribution of $z_n$ as $p(z|a_n)$. Once a new test instance comes, the quantity $KL(q(z|x)|p(z))$ is calculated, the class label corresponding to the smallest divergence will be assigned to the test instance. 

\XS{If we want to force the classifier to learn something that make sense to human, we can use the vgmm-vae (from sun\&gossmann 2019) to create pseudo subdomains, then run DIVA on it. In this case, we force the classifier also to abandon those random features which only correlate to the "true feature", we expect in this case the classifier could generalize. comment?}





==> sec_examples.tex <==
\subsection{Examples of hyperparameters in machine learning}
\subsubsection{From linear regression to Generalized Additive Model (GAM)}
\begin{figure}
    \centering
\includestandalone[width=0.9\textwidth]{tex/tikz/tikz_ridge_regression}
\caption{Ridge regression: $\arg\min_{\theta}\left(||Y - X\theta||^2 + \lambda||\theta||^2\right)$}
\label{fig:ridge_regression}
\end{figure}
\begin{figure}
    \centering
\includestandalone[width=0.9\textwidth]{tex/tikz/tikz_lasso_regression}
\caption{Lasso regression: $\arg\min_{\theta}\left(||Y - X\theta||^2 + \lambda|\theta|\right)$ which correspond to a Laplace prior $Laplace(\theta, \mu, \gamma)=\frac{1}{2\gamma}\exp(-\frac{|x-u|}{\gamma})$}
\label{fig:lasso_regression}
\end{figure}
Ridge regression as depicted in Figure~\ref{fig:ridge_regression} and Lasso regression as depicted in Figure~\ref{fig:lasso_regression} are two common examples of use of regularization term in the objective function in machine learning, where the coefficient $\lambda$ is the hyperparameter which balances between underfitting and overfitting of data. 
Generalized Additive Model (GAM) is a family of Structural Risk Minimization (SRM) where the loss function is a sum of likelihood and regularization term with similar penalty or regularization term. 

When viewed from a Bayesian perspective, ridge regression correspond to a Gaussian prior on the model parameters, while Lasso regularization correspond to a Laplacian prior on the model parameters. The problem is if the mentioned prior is appropriate to model the data in any application. Intuitively, in the data generation process of a Bayesian model corresponding to the data set has a prior which looks different compared to a diamond (for Lasso regularization) or disk (for ridge regularization), it is not possible to have a perfect fit in terms of the shapes of contours of prior distribution on the parameters.

\subsubsection{VAE model family}
Despite the surge of the VAE family model since it was first proposed in 2014, little attention has been paid that the most widely used VAE version is only \textbf{semi-Bayesian}. It is in principle possible to put the neural network weight distribution into the ELBO calculation, which this work tries to utilize as a handle to tune the model. In variational-EM algorithm, the hyper-hyper-parameters are estimated through an Expectation-Maximization like process. In a decentralized setting, due to lack of data, we can not carry out EM directly, can we use Bayesian optimization to approximate a better hyper-prior?

\paragraph{Beta-VAE} 
Beta VAE try to reduce the capacity of the latent representation in order to force the encoder to learn a reasonable representation, otherwise, the neural network might learn something random which has a correlation only with the "true feature". 
\begin{align}
\log p(x) = \underbrace{E_q \left[\log p_{\theta}(x|z)\right]}_{\text{"reconstruction"}} - \beta \underbrace{D_{KL}(q_{\phi}(z \mid x)|| p(z))}_{regularization} + \underbrace{D_{KL}(q_{\phi}(z \mid x) || p(z \mid x))}_{\text{minorization gap}}	
\end{align}
When the latent layer has big capacity, $q(z\mid x)$ can be rather flexible, the ELBO's regularization part function as an "effective capacity" controller: Since the prior $p(z)$ is Gaussian, which is isotropic, the regularization term will force the learned latent representation towards independent with respect to each dimension, so each latent dimension will represent a "meaning". Furthermore, the regularization term forbid the latent representation to be too flexible, thus the latent representation is forced to learn something that really characterize the data generation factor, which leads to the disentanglement effect. Once the latent representation reveals disentanglement, it can lead to robust classification, even with linear classifiers, since the classification now relies on human interpretable features.
%\NC{there is a paper about disentanglement and domain generalisation. DIVA: Domain Invariant Variational Autoencoders}
\paragraph{Vamprior}\cite{tomczak2017vae}
\begin{align}
ELBO(x;\mu, \phi, \theta) = E_{\epsilon}\left[\log p_{\theta}(x\mid z) + \underbrace{\log \frac{1}{K}\sum_{k=1}^{K}p_{\lambda_k}(z)}_{\text{mixture of Gaussian Prior}} - \log q_{\phi}(z|x) \right]
\end{align}


\begin{align}
ELBO(x;\mu, \phi, \theta) = E_{\epsilon}\left[\log p_{\theta}(x\mid z) + \underbrace{\log \frac{1}{K}\sum_{k=1}^{K}q_{\phi}(z|\mu_k)}_{\text{prior coupled with posterior}} - \log q_{\phi}(z|x) \right]
\end{align}

\XS{We want a latent representation that is robust for classification, like disentanglement, not sure in this case, the marginal likelihood is ever important?}

\XS{What is the real difference theoretically between MOG prior and Vamprior,  in term of gradient term? when you compare equation(25) with (26) in \cite{tomczak2017vae}}

%\verb|self.idle_input =Variable(torch.eye(self.args.number_components, self.args.number_components))|

%\verb|X = self.means(self.idle_input)| $K\times K$ to K $\times$ real image size

%\verb|z_p_mean, z_p_logvar = self.q_z(X)  # K(component) x M(latent dimension) |

\paragraph{Implict prior} \cite{takahashi2019variational}"rewrite this KL
divergence that contains the high-dimensional density ratio
into the sum of the analytically calculable term and the low dimensional density ratio term, to which the density ratio
trick is applied.  "
\subsubsection{Life Long Learning}
\paragraph{Life Long Learning}\cite{de2019continual}
%"Artificial neural networks thrive in solving the classification problem for a particular rigid task, where the network resembles a static entity of knowledge, acquired through generalized learning behaviour from a distinct training phase. However, endeavours to extend this knowledge without targeting the original task usually result in a catastrophic forgetting of this task. Continual learning shifts this paradigm towards a network that can continually accumulate knowledge over different tasks without the need for retraining from scratch, with methods in particular aiming to alleviate forgetting. We focus on task-incremental classification, where tasks arrive in a batch-like fashion, and are delineated by clear boundaries. Our main contributions concern 1) a taxonomy and extensive overview of the state-of-the-art, 2) a novel framework to continually determine stability-plasticity trade-off of the continual learner, 3) a comprehensive experimental comparison of 10 state-of-the-art continual learning methods and 4 baselines. We empirically scrutinize which method performs best, both on balanced Tiny Imagenet and a large-scale unbalanced iNaturalist datasets. We study the influence of model capacity, weight decay and dropout regularization, and the order in which the tasks are presented, and qualitatively compare methods in terms of required memory, computation time and storage."
\XS{To Read: Learning bounds \cite{blitzer2008learning}, Unsupervised domain adaptation \cite{ganin2014unsupervised}}



==> sec_learning_theory.tex <==
\section{Statistical Learning theory}
\paragraph{Generalization Decomposition}
Let $\mathcal{D}$ represent the true data distribution, $S$ represent the training sample. Let $L_S(\cdot)$ evaluate a hypothesis with respect to sample $S$, let $L_{\mathcal{D}}(\cdot)$ represent the true risk evaluated on a hypothesis. 
Let $h_S \in \mathcal{H}$ denote the best hypothesis returned by the learning process via the limited size training sample $S$, i.e. $L_{S}(h)\ge L_S(h_s) \forall h \in \mathcal{H}$ let $h^{*}$ denote the best hypothesis with the lowest risk with respect to the whole distribution (i.e. the smallest possible generalization error), i.e. $L_{\mathcal{D}}(h^{*})\le L_{\mathcal{D}}(h) \forall h \in \mathcal{H}$. We can decompose our generalization error into two parts. 
\begin{align}
 &L_{S}(h_S)-L_{\mathcal{D}}(h^{*}) = \\
 &L_{S}(h_S)- L_{\mathcal{D}}(h_S)+  L_{\mathcal{D}}(h_S)-L_{\mathcal{D}}(h^{*})  \ge 0
\end{align}
$L_{S}(h_S)- L_{\mathcal{D}}(h_S)$ is the error due to the sample $S$ gives us the wrong information about the fitness of hypothesis $h_S$, and  $L_{\mathcal{D}}(h_S)-L_{\mathcal{D}}(h^{*})  \ge 0$ measures how far the $h_S$ is to $h^{*}$ in terms of the true objective function. 

\paragraph{Error decomposition}
\begin{align}
    L_{\mathcal{D}}(h_S) &= \min_{h\in \mathcal{H}}L_{\mathcal{D}}(h) + \left(
    L_{\mathcal{D}}(h_S)-\min_{h \in \mathcal{H}} L_{\mathcal{D}}(h)
    \right)\\
    &=L_{\mathcal{D}}(h^{*}_H) + \left(L_{\mathcal{D}}(h_S) -L_{\mathcal{D}}(h^{*}_H)\right)
\end{align}
For neural network, we can assume $\min_{h\in \mathcal{H}}L_{\mathcal{D}}(h)=0$. 
\paragraph{Uniform converging $\epsilon$-representative training set with respect to hypothesis class $\mathcal{H}$} Due to limited training data, the objective function we used to train the neural network is constructed by the finite set of training data, while the true risk we care about is with respect to the whole distribution, thus resulting in the discrepancy between the true objective and the approximated objective via the data. Suppose we construct a sampling strategy with a sample size limit $m_H$, s.t. with sample size bigger than this limit sample size, we can ensure that evaluating each hypothesis with respect to the training dataset induced error function and the true distribution will only result in a bounded discrepancy. Mathematically, let $L_S(\cdot)$ denote the error evaluated upon the training set $S$, $\mathcal{D}$ denote the true distribution, $L_{\mathcal{D}}(\cdot)$ denote the risk with respect to the true distribution. 

$\forall h \in \mathcal{H}$, if $|S|>m_H$, then $|L_S(h)-L_{\mathcal{D}}(h)|\le \epsilon$
%}

\paragraph{PAC Learnable} With probability at least $1-\delta$,
one has $L_{D, f}(h_S)\le \epsilon$, 

\begin{align}
C_1\frac{d+\log(1/\delta)}{\epsilon^2}\le m_{\mathcal{H}}^{UC}(\epsilon, \delta)\le  C_2\frac{d+\log(1/\delta)}{\epsilon^2}   
\end{align}
\paragraph{Growth Function} Let $\mathcal{H}$ be a hypothesis class, $S$ be the training set with size $m$, let $\mathcal{H}_S$ be the effective VC dimension of $\mathcal{H}$ restricted by training set $S$. Then  $\tau_{\mathcal{H}}(m)=\max_{|S|=m}|\mathcal{H}_S|$. The growth function quantifies the maximum "volume" of behaviors of a hypothesis class $\mathcal{H}$ can have on a training set of size $m$.  If the training set size is smaller than the VC dimension of $\mathcal{H}$, then since the training set can always be shattered, then $H_S=2^m$. It is interesting to know when our training dataset increases, how fast the growth function grows. 
\paragraph{Sauer-Shelah-Perles Lemma}
Let $VCdim(\mathcal{H})=d$, when $m=|S|>d+1$, let $e=2.17$, then
\begin{align}
\tau_{\mathcal{H}}(m)\le (em/d)^d
\end{align}, which is a polynomial growth with respect to training dataset size $m$.

\paragraph{Concentration inequality}
If VC dimension is less than infinity, e could use the Sauer-Shelah-Perles Lemma to show that the growth function is polynomial with respect to the VC dimension.
Since with probability $1-\delta$, we have,
%\begin{align}
%    Pr\left(|L_{\mathcal{D}}(h)-L_S(h)|&\le \frac{4+\sqrt{\log (\tau_{H}(2m))}}{\sigma\sqrt{2m}}\right)\\
%    &=\frac{4+\sqrt{d\log (2em/d)}}{\sigma\sqrt{2m}}
%\end{align}
which decreases as the training sample size $m$ increases.

If we have access to a validation set
\begin{align}
&Pr\{|L_V(h)-L_{\mathcal{D}}(h)|\le \sqrt{\frac{log(2/\delta)}{2m_v}}\}>1-\delta\\
&|V|=m_v\\
&V=\{(x,y)|x,y \sim \mathcal{D}\}
\end{align}

==> sec_open_question.tex <==
\section{Open questions}
\subsection{Search of feedback control signal $\mu^{(k)}$ and $b^{(k)}$}
How can we improve the chance that a reg-pareto operator exists for quite a few steps? 

Let $\theta$ be embedded in $\mathbb{R}^p$, we use $g(\cdot)$ to represent the subgradient of $L(\theta, \mu)$ w.r.t. $\theta$, $H(\cdot)$ to represent the Hessian of $L(\theta, \mu)$ w.r.t. $\theta$, let $\hat{H}(\cdot)$ be a positive definite approximation to $H(\cdot)$. Let $\sigma_{max}(\cdot)$ denote the biggest eigenvalue of a matrix and $\sigma_{min}(\cdot)$ denote the smallest one. Let $d(\cdot)\in \mathbb{R}^p$ define a direction for $\theta$, e.g. via a one dimensional eigen-subspace. 

\begin{definition}
A local sublevel set $S_L(\theta^{*}, \epsilon, \delta)$ w.r.t. loss $L(\cdot)$ and $\theta^{*}$, with constant $\epsilon$ and $\delta$ is a set
\begin{equation}
S_L(\epsilon, \delta)=\{\theta |0\le L(\theta, \cdot) -L(\theta^{*}, \cdot) \le \epsilon ~\&~ |\theta-\theta^{*}| \le \delta \}  
\end{equation}
\end{definition}
\begin{conj}
For neural network, with respect to any local minimum $\theta^{*}$, $\exists \epsilon, \delta$ s.t. $S_L(\epsilon, \delta)$ defines a connected topology (at least when both $\epsilon$ and  $\delta$ are small enough).    
\end{conj}
\begin{conj}    
Suppose we are at a local minimum of $L(\theta, \mu)$ with respect to $\theta$. If $\hat{H}(\cdot)$ is a good approximation to $H(\cdot)$, then $d(\sigma_{max}(\hat{H}))$ is a better direction than $d(\sigma_{min}(\hat{H}))$ in finding the next reg-pareto descent operator.   

Along a direction $d(\cdot)$ that is mostly composed of subspaces corresponding to small eigenvalues of $H(\cdot)$ is difficult to find the next reg-pareto descent operator.   
\end{conj}
\begin{prop}
A characterization for reg-pareto descent operator $\mathcal{A}$ is $\mathcal{A}$ moves $\theta^{(k)}$ in a direction that descent  $\ell(\cdot)+\mu^{(k+1)}R(\cdot)$ but ascent $\ell(\cdot)+\mu^{(k)}R(\cdot)$, if an algorithm is able to fix $\theta^{(k)}$ to be a local minimum, then by moving "small" enough along the descent direction of  $\ell(\cdot)+\mu^{(k+1)}R(\cdot)$,  $\mathcal{A}$ is found. 
\end{prop}
\begin{remark}
How to ensure "small"?   
\end{remark}
\begin{definition}
A shallow local minimum is an $\theta^{*}$ s.t. $S_L(\theta^{*}, \epsilon, \delta)$ has small volume for its connected component with fixed $\epsilon, \delta$
\end{definition}
\begin{remark}
Since we have in general no control over the behaviour of the low level controller $\mathcal{O}(\cdot)$ (e.g. ADAM), we should avoid setting $\theta^{(k)}$ in our algorithm to be shallow local minimum.\end{remark}
\begin{conj}
one could find $\mathcal{A}$ by optimizing a direction $d(\cdot)$ s.t. it aligns with both the descent direction of $\ell(\cdot)+\mu^{(k+1)}R(\cdot)$ and descent direction of $R(\cdot)$ by proximal gradient.
\end{conj}

\subsection{Open questions}
\begin{itemize}
\item what is a good characterization of local minimum with respect to an optimizer $\mathcal{O}(\cdot)$? i.e. when do I know 
if it is easier to find a reg-descent optimizer? (Hessian has good condition number?) 
\item Intuitively, a bigger increase in $\mu$ will make it easier for finding the next reg-descent condition, could someone offer a proof?  
\item if $\mu$ is very large, how to ensure $\ell(\cdot)+\mu R(\cdot)$ won't have too big gradient? (of course one could curb the gradient or set a maximum value for $\mu$) (nutan)
\item How to characterize the volume of $S_L(\epsilon, \delta)$
\item How to design $\mu^{(k)}$ in a model predicative way, s.t. a reg-pareto optimizer can be found for a long sequence? 
\end{itemize}

==> sec_rfms_intro.tex <==
Machine learning faces the challenge of distribution shift~\cite{akuzawa2019adversarial} and data privacy problem~\cite{long2017deep, sun2019high, Konecny2016, federatelearnCommuni, Brendan2017}. \NC{more reasons: computation and real-time requirements do not allow to retrain the model. For instance, an app needs to predict an object from a figure with a background which is unseen in the training data.}

While most works focus on federated learning~\cite{federatelearnCommuni}, by aggregating local updates towards a shared central model, in some biomedical applications, it might be the case some data sites are not able to provide local updates, especially in a communication intensive manner. Restrictive Federated Model Selection (RFMS)~\cite{sun2019high} applies when the remote data site can only be used for prediction, in which case, the performance of a sent model to the remote site could be used as feedback information to tune a better model trained locally. The tuned model by untilizing local and remote performance information has been shown empirically to work under the data distribution of both local and remote data sites.

In RFMS, there are three types data sites. The openbox $D_{ob}$ refer to data site with unrestricted data acess, the curator $D_{cu}$ refer to data site that can offer feedback signal to the model in the form of performance estimator, and lockbox $D_{lb}$ refer to data site that can not offer assistance to the machine learning process but still wants benefit from the model, i.e.~the model should generalize well to $D_{lb}$ as well. In this work, we inherit their terminology. The learning process of RMFS is depicted in Figure~\ref{fig:rfms}.
\begin{figure}
	\centering
	\includegraphics[scale=0.3]{fig/rfms.png} 
        \caption{RFMS:~\protect\input{caption_rfms}}
	\label{fig:rfms}
\end{figure}


However, in their work, only vector data types with machine learning models like support vector machine is considered. In this work, we condiser image data with neural networks.
We call this learning scenario \textbf{partial shot probing learning} because we can only get the prediction performance from remote data site, instead of sample data. From a broader category, we name this problem \textbf{domain generalization with restrictive data access}.





==> sec_rfms_pgm.tex <==
\subsection{Extending to multiple data sites}
A probabilistic graphical model for this can be shown in Figure~\ref{fig:pgm_rfms_multi_datasite} %where we have overloaded the usual plate representation for number of variables for undirected cliques. There are three types data site openbox $D_{ob}$, curator $D_{cu}$ and lockbox $D_{lb}$, each generated by a different Data Generation Process corresponding to different domains. The observable $S$ are the prediction score like accuracy or brier score. $\theta$ represent parameters for a prediction model, while $\phi$ represent associated hyper-parameters.

\begin{figure}
	\centering
	\includegraphics[scale=0.9]{tikz_pgm_hyper_parameter_towards_bayes_multi_datasite} 
        \caption{\protect\input{caption_pgm_rfms_multi_datasite}}
	\label{fig:pgm_rfms_multi_datasite}
\end{figure}

We are interested in the following research questions:
\begin{enumerate}
  %\item What would be a good measure on the generalization ability of the domain generalization problem? In other words, what is a good evaluation scheme for \textbf{Domain Generalization with restrictive data access}? \AG{Once the whole system is trained evaluate the task performance on previously unseen data (i.e., freeze the model, open up $D_{lb}$, and check performance on task of interest on $D_{lb}$)? Or is there more nuance that I don't see?}
  \item Can we find a set of low dimensional hyper-parameter to fine tune a generative model like VAE such that it could generalize to different distributions?
  \item In terms of learning theory \cite{redko2019analysis}, it is possible to quantify to what extent could a model generalize to a never seen data site $D_{lb}$ if we only train upon data from a single data site. \AG{Ideally, this should be a function of the amount of distribution shift between the seen and unseen datasets, and also take properties of the data distribution and the task into account. I think that focusing on the ``worst case'' may not be the best way, because the theoretical results will be very pessimistic.} Now with acess to a scalar valued performance estimator $S$, is it possible to simply use $S$ as feedback signal to tune the above-mentioned hyper-parameters to achieve better generalization bound?
	\item If the problem is simplified to only get unlabeled data or mixed unlabeled and small number of labeled data from remote datasite, by using Unsupervised Data Augmentation \cite{xie2019unsupervised}, what would be the result? \NC{1, mixup by Zhang 2017 is also a good and simple data augmentation method. 2, if the problem is simplified as this, it is domain adaptation instead of domain generalisation. In this case, perhaps we can try the idea which I proposed: we could first try to use the posterior of the first task, as the prior for the second task}
\end{enumerate}
\AG{Some further questions:\\ What is the effect of the number of data sources with restricted access? Does the model generalization improve the more data sources we have? Is there something like a minimal required number of data sources to achieve a desired level of model generalizability, and what is the relationship to the number of training samples?\\ Related to continual/life-long learning: Can this methodology address the scenario when data sources (with restricted access) are continuously added and/or removed as time goes on? What is the proper way to continue training or retrain once a new data source (with restricted access) becomes available? In real life situations, the data within previously available data sources may change/grow/shrink too as time goes on.}




==> sec_setpoint_model_sel.tex <==
\subsubsection{Multi-objective setpoint based model selection}\label{sec:msel_setpoint}
%Since validation accuracy could reach a very high value (e.g. 1.0) when the validation set is used for model tuning or hyperparameter selection, simply selecting model based on improvements of validation accuracy will stop the training pre-maturely, before the output loss $R$ could track the setpoint. Nonetheless, if we characterize an improved model as one with at least equal validation performance, there is a possibility that the latest model will consistently be chosen. However, this does not guarantee superior test accuracy.
%To address the issue, we make two amendments to the conventional model selection based on validation accuracy: Firstly, we implement a top-2 criterion, where we retain the models with the two highest validation accuracies. According to the top-2 criterion, a new model is considered superior if its validation accuracy surpasses that of the model with the second-best validation accuracy.
%Secondly, 
In general, the feasibility in \Cref{eq:feasibility_r} becomes more difficult to be met each time the setpoint $b$ shrinks. After several setpoint shrinkages, the difficulty of attaining the feasibility can lead to an oscillating behavior of $R(\cdot)$ around the setpoint with uncontrolled amplitude, as shown in \Cref{fig:dyn_pacs_diva_fbopt}. To circumvent this behavior, the up-to-event best model is selected at the last setpoint shrinkage.  
%In between two setpoint shrinkage events, $R(\cdot)$ does not Pareto dominate the previous setpoint, other model selection criteria like validation set performance can 
% TODO: the last shrinkage event did dominate the previous setpoint, so model selection can be non-dominant based (validation acc) or dominance based (pure multi-loss sel)







%which we term hindsight model selection.
%, where the output $R(\cdot)$ is still bounded by the setpoint. %This model selection criteria avoids the situation at later optimization iterations where feasibility can not be ensured anymore, 
%This is crucial as there may be instances where the new setpoint is unattainable. Constraining only when the output $R(\cdot)$ enters the feasibility region \cref{eq:feasibility_r} gives us a deterministic and multi-objective criterion to select models, such that \cref{eq:feasibility_r} is satisfied.

==> sec_solution_failed.tex <==
\subsection{Potential Solutions}
For simplicity, we first consider classification task.
In Figure~\ref{fig:arch}, we showed two possible ways of implementing the Bayesian Restrictive Federated Partial Shot Learning. We use circle to represent random variables, use cube to represent a neural network, and use square to represent the constant and variables in a computational graph. The arrows represent either input or normalizing flows \cite{bibid}. The output of the neural network are "reconstructed" image and prediction label, ie. for semisupervised learning.

\subsubsection{Simple data augmentation won't work}
In (b) of Figure \ref{fig:arch}, inspired by Universal Value Function Approximator \cite{schaul2015universal}, we use a low dimensional input $v$ to map to the same dimension with the image $X$, which equivalently add batchsize to the training of VAE. $v$ serves as constant in the computational graph, by could be tuned by Bayesian Optimization which kind of serves as a "sufficient statistic" for the remote data site that can not be seen. \textbf{However, the weights associated with $v$ in this case will compensate $v$ away in the loss, which result in no difference as not adding $v$ at all.}
\XS{how UVFA \cite{schaul2015universal} avoid this problem?}

\subsubsection{Tuning vamprior}
In (a) of Figure \ref{fig:arch}, we use a modified vampPrior \cite{tomczak2017vae}. The auxilliary input in standard vampPrior is the $K$ $u_k$ input, which can be learned by backpropagation to form a prior that is closest to the posterior. Inspired by InfoGan \cite{chen2016infogan}, we split the auxilliary input into two components, the original $u_k$ which can be learned with Backpropagation, and the constant input $v$ which remains constant in the backpropogation, but could be tuned with Bayesian Optimization. In this way, $v$ could be learned to represent the remote data distribution.
\begin{align}
	\mu_k = M_{KX} \times (VAR_{EYE}(K) + CONST_{diag}(K))
\end{align}
or
\begin{align}
\mu_k = M_{KX} \times (VAR_{EYE}(K) \times CONST_{diag}(K))
\end{align}

$CONST$ is constant with respect to back propagation, the same size matrix as $VAR_{EYE}(K)$ (Variable of size $K \times K$). $M_{KX}$ is the neural network that maps Variable $PH_{EYE}(K)$ to a real image size.

\textbf{question is what should be the form of $CONST$?  A full matrix or a diagnal one? which must be easy to search. As discussed, will this added term be "adapted way"?}
\XS{infoGAN \cite{chen2016infogan} also split the noise into two parts, why the variables in infoGAN is not adapted away?}
\AG{Related to XS question above. From the InfoGAN paper: ``rather than using a single unstructured noise vector, we propose to decompose the input noise vector into two parts: (i) $z$, which is treated as source of incompressible noise; (ii) $c$, which we will call the latent code and will target the salient structured semantic features of the data distribution.'' I think neither $z$ nor $c$ are ``adapted away'' because neither variable is constant. $z$ is noise (so, resampled in every iteration) and $c$ is in a sense part of a latent representation that is learned.}
\XS{@AG, I think you are right}

\subsubsection{Tuning Gaussian Mixture Prior}
A third option is to tune the Gaussian Mixture prior in place of the  standard Gaussian prior which is hopefully representing a joint prior between the local and remote data site. 
\begin{align}
ELBO(x;\mu, \phi, \theta) = E_{\epsilon}\left[\log p_{\theta}(x\mid z) + \underbrace{\log \frac{1}{K}\sum_{k=1}^{K}p_{\lambda_k}(z)}_{\text{backprop mixture Prior}} + \underbrace{\log \frac{1}{K}\sum_{k=1}^{K}p_{\beta_k}(z)}_{\text{constant mixture prior}} - \log q_{\phi}(z|x) \right]
\end{align}
\AG{What is the difference between $p_{\lambda_k}(z)$ and $p_{\beta_k}(z)$ in the above equation?}
\XS{@AG, on is the mean and variance to be optimized with BP, the other is fixed mean and variance}
\begin{figure}
\includegraphics[scale=0.5]{fig/partialShotVampPrior.pdf} 
\caption{Architecture of two partial shot RFMS \NC{basically, it is hyperparameter search. If we are lucky, we may get a good hyperparameter. However, the causal relationship between the domain generalisation and these hyperparameters is missing.}
\XS{@NC, take conjugate prior as an example, the posterior is the same family of distribution as the prior, in which case,the prior parameters correspond to pseudo observations. In Figure (a), we are searching for pseudo observations, would the pseudo observations be a n appropriate causal factor to generalization?}
}
\label{fig:arch}
\end{figure}

\TODO{use mixture of Gaussian instead of vamprior to do the tuning}

\subsubsection{Tuning the classifier neural network weights distribution}
As mentioned before, most VAE versions are semi-Bayesian. We extend VAE to full Bayesian by considering the distribution of neural network weight. For a classification task, we focus on the classifier weight prior.


==> sec_vae.tex <==
In a Bayesian setting, however, we usually try to model the data generative process. For example, in variational auto-encoding for semi-supervised learning as shown in the probabilistic graphical model in Figure~\ref{fig:m2}, we model latent representation of individual observation (Note that VAE is not fully Bayesian which still falls into the frequentist approach category, but we just use this empirical Bayesian approach of VAE to illustrate the idea of data generation process). The observed class label $y$ explains the class-label induced variance of the image $X$, while the latent variable $z_d$ explains the domain information. Note however, given arbitrary data, we can not figure out what is the true data generating process, a VAE only gives us a good guess of the true model which explains the data well enough.

\begin{figure}[h!]
	\centering
	\includegraphics[scale=0.9]{tex/tikz/tikz_m2.pdf} 
	\caption{Semi-supervised VAE}
	\label{fig:m2}
\end{figure}


==> sec_vae_fundamental.tex <==
\section{Prerequisite}
\paragraph{VAE}
VAE use latent variable model to build more complicated distribution model for data $X$. Let $Z$ denote the latent variable. Use $\theta$ to denote the decoder network $G$ which specifies the conditional distribution $p_{\theta}(x|z)$ by two heads. The posterior $p(z|x) = \frac{p(z)p(x|z)}{\int p(\tilde{z})p(x|\tilde{z})d\tilde{z}}$ is intractable. Use variational distribution $q_{\phi}(z|x)$ to replace the intractable model posterior, represented by encoder network $Q$, where $z$ is reparameterized by prior distribution over $\epsilon$, which get mapped to distribution parameter of $z$. The objective function of VAE is Evidence ($\int_z p(x,z)dz$) Lower Bound (ELBO), which is

\begin{align}
	\log p(x) &= \log p(x, z) - \log p(z|x) \underbrace{+ \log q_{\phi}(z|x) - \log q_{\phi}(z|x)}_{\text{plus minus trick}}\\
	\log p(x)&= \log p(x)\int_z  q(z\mid x)dz=\int_z \log p(x) q(z\mid x)dz = E_q \left[\log p(x) \right] \\
	&= E_q \left[\log p(x,z)\right] \underbrace{- E_q \left[\log p(z|x)\right] + E_q \log q_{\phi}(z|x)}_{\text{minorization gap}} - E_q \log q_{\phi}(z|x)\label{eqn:between}\\
&= E_q \left[\log p(z)+ \log p(x \mid z)\right] \underbrace{- E_q \left[\log p(z|x)\right] + E_q \log q_{\phi}(z|x)}_{\text{minorization gap}} - E_q \log q_{\phi}(z|x)\\
	&= E_q \left[\log p(x \mid z)\right] - E_q \left[\log \frac{q_{\phi}{(z\mid x)}}{p(z)}\right] + \underbrace{E_q \left[\log \frac{q_{\phi}{(z\mid x)}}{p(z \mid x)}\right]}_{\text{minorization gap}} 
\end{align}
With Jenson inequality, we have

$\underbrace{E_q \left[\log \frac{q_{\phi}{(z\mid x)}}{p(z \mid x)}\right]}_{\text{minorization gap}} = \underbrace{D_{KL}(q_{\phi}(z \mid x) || p(z \mid x))}_{\text{minorization gap}}=\underbrace{E_q \left[-\log \frac{p(z \mid x)}{q_{\phi}{(z\mid x)}}\right]}_{\text{minorization gap}}>=\log \underbrace{E_q \left[\frac{p(z \mid x)}{q_{\phi}{(z\mid x)}}\right]}_{\text{minorization gap}}=0$

Equation \ref{eqn:between} can also be written as
\begin{align}
	\log p(x)&= -D_{KL}(q_{\phi}(z|x)||p(x,z))+\underbrace{- E_q \left[\log p(z|x)\right] + E_q \log q_{\phi}(z|x)}_{\text{minorization gap}} \\
	&=-F(\phi,theta)+\underbrace{- E_q \left[\log p(z|x)\right] + E_q \log q_{\phi}(z|x)}_{\text{minorization gap}}
\end{align}

if we define
\begin{align}
	ELBO(\phi, \theta) &= -F(\phi,theta)\\
	&=E_q \left[\log p_{\theta}(x \mid z)\right] - E_q \left[\log \frac{q_{\phi}{(z\mid x)}}{p(z)}\right]
\end{align}
so
\begin{align}
	\log p(x) = ELBO(\phi, \theta) +  \underbrace{D_{KL}(q_{\phi}(z \mid x) || p(z \mid x))}_{\text{minorization gap}}	
\end{align}
To optimize the ELBO with minibatches, $q_{\phi}(z \mid x)$ is represented by parameters of fixed distribution from seed distribution $p(z)$. The parameters are mapped from $x$ through encoder network $\phi$, which through pre-sampled $\epsilon$ following $p(z)$, are mixed into the final latent value. $\log p_{\theta}(x\mid z)$ is represented by another distribution (if x is continuous, then is Gaussian), with its parameters mapped by the decoder network. In this case, the expectation with respect to the Variational distribution could be approximated by Monte Carlo sampling.
 
If we majorize the evidence $\log p(x)$, 
\begin{align}
	&D_{KL}(q_{\phi}(z \mid x) || p(z \mid x))\\
	=&- E_q \left[\log p(z|x)\right] + E_q \log q_{\phi}(z|x)
\end{align} 

\paragraph{GAN compared to VAE} GAN \cite{goodfellow2014generative} trains a discriminator and generator network simultaneously via the mini-max game. The discriminator is trained to distinguish data from samples and generators, while the generator is trained to mimic the samples data to deteriorate the performance of the discriminator. Auxiliary Classifier GAN (ACGAN) \cite{odena2017conditionaL} augment the input of the generator network with the class label, and augment the output of the discriminator network with a classification output. Both the discriminator and the generator are trained to recover the classification output at the discriminator output, while they optimize against the ability of the discriminator to tell apart the fake samples. 

\paragraph{Amortization Gap}
\cite{cremer2018inference}
\paragraph{Info-VAE}
\paragraph{Info-GAN}
\paragraph{Conditional Variational Autoencoder (CVAE)}




==> sec_val_learning_theory.tex <==
The validation set $\mathcal{D}_{val}$ is used due to
\begin{align}
&Pr\left\{\left|L_{\mathcal{D}_{val}}(h)-L_{\mathcal{D}}(h)\right|\le \sqrt{\frac{log(2/\delta)}{2m_v}}\right\}>1-\delta\\
&|\mathcal{D}_{val}|=m_v\\
&\mathcal{D}_{val}=\{(x,y)|x,y \sim \mathcal{D}\}
\end{align}
However, in reality, it is usually not possible to get a validation set that follows the true distribution $\mathcal{D}$. Also, the validation set accuracy might saturate to be 1 which makes models indistinguishable.

==> subsec_multi_obj_msel.tex <==
% \section{Multi-objective setpoint based model selection}\label{sec:msel_setpoint}
% %Since validation accuracy could reach a very high value (e.g. 1.0) when the validation set is used for model tuning or hyperparameter selection, simply selecting model based on improvements of validation accuracy will stop the training pre-maturely, before the output loss $R$ could track the setpoint. Nonetheless, if we characterize an improved model as one with at least equal validation performance, there is a possibility that the latest model will consistently be chosen. However, this does not guarantee superior test accuracy.
% %To address the issue, we make two amendments to the conventional model selection based on validation accuracy: Firstly, we implement a top-2 criterion, where we retain the models with the two highest validation accuracies. According to the top-2 criterion, a new model is considered superior if its validation accuracy surpasses that of the model with the second-best validation accuracy.
% %Secondly, 
% In general, the feasibility in \Cref{eq:feasibility_r} becomes more difficult to be met each time the setpoint $b$ shrinks. After several setpoint shrinkages, the difficulty of attaining the feasibility can lead to an oscillating behavior of $R(\cdot)$ around the setpoint with uncontrolled amplitude, as shown in \Cref{fig:dyn_pacs_diva_fbopt}. To circumvent this behavior, the up-to-event best model is selected at the last setpoint shrinkage.  





==> table_hyperpar.tex <==
 \begin{table*}[]
 \begin{tabular}{rllrrrr}
\toprule
 Configuration &                Method & Model &  k\_i\_gain\_ratio &  $\mu_{clip}$ &  $\gamma_d$ &  $\gamma_y$ \\
\midrule
0 &          diva\_fbopt\_a &  diva &            0.25 &      1.0 &       -- &       -- \\
1 &          diva\_fbopt\_a &  diva &            0.25 &     10.0 &       -- &       -- \\
2 &          diva\_fbopt\_a &  diva &            0.25 &    100.0 &       -- &       -- \\
3 &          diva\_fbopt\_a &  diva &            0.25 &   1000.0 &       -- &       -- \\
4 &          diva\_fbopt\_a &  diva &            0.55 &      1.0 &       -- &       -- \\
5 &          diva\_fbopt\_a &  diva &            0.55 &     10.0 &       -- &       -- \\
6 &          diva\_fbopt\_a &  diva &            0.55 &    100.0 &       -- &       -- \\
7 &          diva\_fbopt\_a &  diva &            0.55 &   1000.0 &       -- &       -- \\
8 &          diva\_fbopt\_a &  diva &            0.85 &      1.0 &       -- &       -- \\
9 &          diva\_fbopt\_a &  diva &            0.85 &     10.0 &       -- &       -- \\
10 &          diva\_fbopt\_a &  diva &            0.85 &    100.0 &       -- &       -- \\
11 &          diva\_fbopt\_a &  diva &            0.85 &   1000.0 &       -- &       -- \\
12 & diva\_feedforward\_full &  diva &              -- &       -- &      1.0 &       -- \\
13 & diva\_feedforward\_full &  diva &              -- &       -- &   1001.0 &       -- \\
14 & diva\_feedforward\_full &  diva &              -- &       -- & 100001.0 &       -- \\
15 &          diva\_default &  diva &              -- &       -- &      1.0 &      1.0 \\
16 &          diva\_default &  diva &              -- &       -- &   1001.0 &      1.0 \\
17 &          diva\_default &  diva &              -- &       -- & 100001.0 &      1.0 \\
18 &          diva\_default &  diva &              -- &       -- &      1.0 &   1001.0 \\
19 &          diva\_default &  diva &              -- &       -- &   1001.0 &   1001.0 \\
20 &          diva\_default &  diva &              -- &       -- & 100001.0 &   1001.0 \\
21 &          diva\_default &  diva &              -- &       -- &      1.0 & 100001.0 \\
22 &          diva\_default &  diva &              -- &       -- &   1001.0 & 100001.0 \\
23 &          diva\_default &  diva &              -- &       -- & 100001.0 & 100001.0 \\
24 &    diva\_fixed\_penalty &  diva &              -- &       -- &      1.0 &      1.0 \\
25 &    diva\_fixed\_penalty &  diva &              -- &       -- &   1001.0 &      1.0 \\
26 &    diva\_fixed\_penalty &  diva &              -- &       -- & 100001.0 &      1.0 \\
27 &    diva\_fixed\_penalty &  diva &              -- &       -- &      1.0 &   1001.0 \\
28 &    diva\_fixed\_penalty &  diva &              -- &       -- &   1001.0 &   1001.0 \\
29 &    diva\_fixed\_penalty &  diva &              -- &       -- & 100001.0 &   1001.0 \\
30 &    diva\_fixed\_penalty &  diva &              -- &       -- &      1.0 & 100001.0 \\
31 &    diva\_fixed\_penalty &  diva &              -- &       -- &   1001.0 & 100001.0 \\
32 &    diva\_fixed\_penalty &  diva &              -- &       -- & 100001.0 & 100001.0 \\
33 &                   erm &   erm &              -- &       -- &       -- &       -- \\
\bottomrule
     \end{tabular}
     \caption{Hyperparameter settings for the different runs in Figure~\ref{fig:benchmark_pacs_diva}.}
     \label{tab:benchmark_pacs_diva_params}
 \end{table*}

==> thm_not_used.tex <==





\begin{corollary}    
\label{remark:globalopt}
Let $\theta_{\mu}:=\arg\min_{\theta}\ell(\theta)+R(\theta)$, then let 
\begin{align}
\theta^{(k)}, \mu^{(k)} \mapsto 
\bar{\theta}^{(k)}=\theta_{\mu^{(k)}}, ~
\theta^{(k+1)}=\theta_{\mu^{(k+1)}}~, \mu^{(k+1)} > \mu^{(k)}    
\end{align}
then $R(\theta^{(k+1)})-R(\bar{\theta}^{(k)}) \le 0$
\end{corollary}

\begin{corollary}    
Starting from an initial parameter configuration $\theta^{(0)}$, 
let $\mu^{(0)}=0$, $\bar{\theta}^{(0)}=\theta_{\mu=0}$. Design a high-level control signal
$\mu^{(k)} > \cdots > \mu^{(1)}>\mu^{(0)}$, such that the evolution of $\theta$ and $\mu$ follows \Cref{def:reg-pareto-slider}. Then the closed loop  behaviour of $\theta$ dynamically corresponds to a descent in $R(\cdot)$. 
\end{corollary}

\begin{remark}
The $\arg\min$ in ~\Cref{remark:globalopt} can be replaced by a local minimum operator.
\end{remark}

\begin{conj}\label{conj:exist}
$\exists s^{(0)}, s^{(1)}, \cdots, s^{(k)}, \cdots$ s.t. ~
\begin{align}
\theta^{(k+1)}&=\mathcal{G}_{\mu^{(k+1)}}^{s^{(k)}}(\theta^{(k)})\\
\mu^{(k+1)}&>\mu^{(k)}
\end{align}
with 
\begin{align}
\theta^{(k)},\mu^{(k)} \mapsto \bar{\theta}^{(k)}={\theta}^{(k)}, \theta^{(k+1)}, \mu^{(k+1)}  
\end{align} satisfying \Cref{def:reg-pareto-slider}.
\end{conj}

\begin{remark}
Conjecture~\ref{conj:exist} indicates if one starts from the current model parameter $\theta^{(k)}$, via several steps of gradient descent like algorithm with respect to $\ell(\cdot)+\mu^{(k+1)}(\cdot)$, one could find a parameter configuration $\theta^{(k+1)}$ that improves $\ell(\cdot)+\mu^{(k+1)}(\cdot)$ over $\bar{\theta}^{(k)}$ but deteriorate $\ell(\cdot)+\mu^{(k)}(\cdot)$ over $\bar{\theta}^{(k)}={\theta}^{(k)}$ 
\end{remark}


==> thm_pareto_slider.tex <==

    


\begin{corollary}\label{corollary:reg-descent}
Let
\begin{align}
\{\theta^{(k+1)}, \bar{\theta}^{(k)}, \mu^{(k+1)}\} \in \mathcal{A}(\mathcal{\ell}(\cdot), R(\cdot);\theta^{(k)}, \mu^{(k)}) 
\end{align} from \cref{def:reg-pareto-slider}
then, 
\begin{align}
R(\theta^{(k+1)})&\le R({\theta}^{(k)})\\
\ell(\theta^{(k+1)})&\ge \ell({\theta}^{(k)}) \\
\ell(\theta^{(k+1)})-\ell({\theta}^{(k)})&\le \mu^{(k+1)}( R(\bar{\theta}^{(k)})  -  R(\theta^{(k+1)}))
\end{align}
%i.e. the training objective in Equation \ref{eq:obj_penalty2} lead to smaller regularization loss $R(\cdot)$ compared to the training objective in Equation \ref{eq:obj_penalty2} on the training data. 
%\begin{proof}
%multiply $-1$ to both sides of \Cref{eq:deteriorate_old_lambda}, add the results to \Cref{eq:improve_new_lambda}, 
%we have
%\begin{equation}
%(\mu^{(k+1)}-\mu^{(k)})R(\theta^{(k+1)})\le (\mu^{(k+1)}-\mu^{(k)})R({\theta}^{(k)})
%\end{equation}
%which implies
%\begin{equation}
%(\mu^{(k+1)}-\mu^{(k)})\left(R(\theta^{(k+1)})-R({\theta}^{(k)})\right)\le 0
%\end{equation}
%Since $\mu^{(k+1)}>\mu^{(k)}$
%\begin{equation}
%R(\theta^{(k+1)})-R(\bar{\theta}^{(k)}) \le 0
%\end{equation}
%Equation~\ref{eq:deteriorate_old_lambda} and ~\ref{eq:improve_new_lambda} gives
%\begin{align}
%&0\le \mu^{(k)}( R({\theta}^{(k)})  -  R(\theta^{(k+1)})) \le \\
%&\ell(\theta^{(k+1)}) -\ell({\theta}^{(k)})  \le  \mu^{(k+1)}( R({\theta}^{(k)})  -  R(\theta^{(k+1)})) 
%\end{align}
%thus $\ell(\theta^{(k+1)})\ge \ell({\theta}^{(k)})$
%\end{proof}
\end{corollary}


\begin{remark}
We have $\bar{\theta}$ here to incorporate the situation when condition does not hold for 1 epoch. 
\Cref{corollary:reg-descent} depicts the situation when we increase $\mu$ sequentially until \Cref{eq:feasibility_r}, we could get a descent sequence of $R(\cdot)$ and an ascent sequence of $\ell(\cdot)$. However, in practice, we observed that this situation does not occur often. In many iterations, we have a joint decrease of $\ell(\cdot)$ and $R(\cdot)$ such that, with the overall effect  $\exists m$ satisfying \Cref{eq:l_decrease}. We summarize such a behavior in Conjecture~\ref{conj:l_decrease} based on \Cref{corollary:ellbound}.

%Additionally, with big enough $\mu$, the dominating $\mu R(\cdot)$ term in the penalized objective function will lock the escape of the system to leave the area where $R(\cdot)$ is relatively small, then the remaining possibility to optimize $\ell(\cdot)+\mu R(\cdot)$ will be a decrease in $\ell(\cdot)$. 
\end{remark}

